Performing Co-Membership Attacks Against Deep Generative Models

In this paper we propose a new membership attack method called co-membership attacks against deep generative models including Variational Autoencoders (VAEs) and Generative Adversarial Networks (GANs). Specifically, membership attack aims to check whether a given instance x was used in the training data or not. A co-membership attack checks whether the given bundle of n instances were in the training, with the prior knowledge that the bundle was either entirely used in the training or none at all. Successful membership attacks can compromise the privacy of training data when the generative model is published. Our main idea is to cast membership inference of target data x as the optimization of another neural network (called the attacker network) to search for the latent encoding to reproduce x. The final reconstruction error is used directly to conclude whether x was in the training data or not. We conduct extensive experiments on a variety of datasets and generative models showing that: our attacker network outperforms prior membership attacks; co-membership attacks can be substantially more powerful than single attacks; and VAEs are more susceptible to membership attacks compared to GANs.

==> theory/diversity_short.tex <==
\subsection{Diversity}
Diversity describes whether the generator can produce different samples~\cite{arora18GAN}. We use a measure called \emph{dispersion} to evaluate the diversity qualitatively. Dispersion with a parameter $k$ is defined as the largest value of closest pairwise distance of $k$ points in the generated data. We show that empirically, dispersion, generalization error, and success rate of membership attack are all closely correlated. When we take random samples from the training data -- the more training data we use, the smaller the generalization gap, the higher dispersion in the generated data.  

We display a distinctive difference between diversity and generalization. We apply our membership attack to choose \emph{adversarial samples}, that are hard to be reproduced in the training phase by an attacker network. When we train a new GANs using only these adversarial samples, compared to a GANs trained by random samples with the same number of training data, we can observe a sharp contrast of diversity versus generalization. The GANs with adversarial sampling shows much higher dispersion, but it is easy to launch membership attacks with a large generalization gap. This shows that high diversity of a generative model cannot immediately guarantee good quality and generalization. Adversarial samples focus too much on corner cases and therefore may not effectively approximate the real distribution. More details about diversity can be found in the appendix \url{https://www.dropbox.com/s/fdlnqtzn58ijolr/supp.pdf}.
